What Blocks My Blockchain's Throughput? Developing a Generalizable Approach for Identifying Bottlenecks in Permissioned Blockchains

Permissioned blockchains have been proposed for a variety of use cases that require decentralization yet address enterprise requirements that permissionless blockchains to date cannot satisfy -- particularly in terms of performance. However, popular permissioned blockchains still exhibit a relatively low maximum throughput in comparison to established centralized systems. Consequently, researchers have conducted several benchmarking studies on different permissioned blockchains to identify their limitations and -- in some cases -- their bottlenecks in an attempt to find avenues for improvement. Yet, these approaches are highly heterogeneous, difficult to compare, and require a high level of expertise in the implementation of the underlying specific blockchain. In this paper, we develop a more unified and graphical approach for identifying bottlenecks in permissioned blockchains based on a systematic review of related work, experiments with the Distributed Ledger Performance Scan (DLPS), and an extension of its graphical evaluation functionalities. We conduct in-depth case studies on Hyperledger Fabric and Quorum, two widely used permissioned blockchains with distinct architectural designs, demonstrating the adaptability of our framework across different blockchains. We provide researchers and practitioners working on evaluating or improving permissioned blockchains with a toolkit, guidelines on what data to document, and insights on how to proceed in the search process for bottlenecks.

==> 04_Methods_Fabric.tex <==
\section{Method and Results}
\label{sec:m&f}

We developed the overall approach by analyzing the experiments described in related work, using the~\ac{dlps} to collect data and~\ac{eda} to identify bottlenecks. We collected a large volume of data on factors influencing node performance, ensuring a comprehensive overview of their resource utilization. After cleaning and validating the data, we used~\ac{eda} in search of irregularities or drops in the blockchain’s performance. Upon identifying these issues, we conducted a detailed examination of the relevant metrics at a finer granularity to determine the root causes of these behaviors.
We divided our analysis into two major components. The first part identifies potential bottleneck candidates by examining the different node resources that can impact their performance. In the second part, we examine the relationship between these candidates and the blockchain’s throughput in varying degrees of resolution, for instance, narrowing down the time window or selection of components.
So far, most enterprise applications seem to have focused on Fabric and Quorum, and related work indicates that the bottleneck analysis of both blockchains is intricate, so we decided to detail our bottleneck identification method for both blockchains. 

For our analysis, we selected a particular experiment for Fabric v2.0, drawing upon the findings of~\cite{guggenberger_-depth_2022} to determine a configuration that seems robust under modifications and extended it to Quorum~v23.4. For Fabric, the network configuration comprised 16~clients, 8~peers, and 4~orderers, with four organizations comprised of two peers each. In contrast, the Quorum configuration consisted of 16~clients and 8~nodes. For both blockchains, we opted for the \ac{raft} consensus mechanism due to its minimal overhead, as previous publications suggest that consensus is not the bottleneck in this case~\citep{guggenberger_-depth_2022, mazzoni_performance_2021}. We conducted the experiment on the AWS~cloud platform (Amazon~EC2), where each node was configured in an independent EC2~instance allocated with 16~vCPUs, 64\,GB~of~RAM, and 1\,Gbps of bandwidth running Ubuntu Server~18.04~LTS~(HVM). 


\subsection{Fabric: Resource utilization}
\label{resource_util}

The initial analysis focuses on understanding the impact of incremental increases in the request rate on the resource utilization of each node. This is achieved by plotting a data point for each node every second during a 14-second time-frame within a 20-second experiment (excluding the initial and final 3~seconds where the ramp-up and ramp-down of \ac{freq} may cause temporary effects), corresponding to different request frequencies (Figure~\ref{fig:Scatter_resources}). This method aims to uncover potential trends and correlations between resource usage and increased \ac{freq}. This initial step already indicates that peers exhibit the highest strain in \ac{CPU} usage, as demonstrated by the maximum utilization percentage across all cores on each node while ordering and client nodes display significantly lower \ac{CPU} utilization rates.


In terms of memory usage, both clients and ordering nodes appear largely unaffected by increases in the request rate. However, peers show signs of impact, albeit without a clear pattern. Regarding network and hardware utilization, client nodes maintain stable performance, whereas peer and orderer nodes demonstrate a moderate correlation between increased utilization and \ac{freq}, but as before, the exact trend is not clear. Note that at this early stage of the analysis, any anomalies could also suggest inaccuracies in the experimental setup. Therefore, it is crucial to eliminate this possibility before conducting a more detailed analysis to determine the structural causes behind these observations. Upon ruling out experimental errors, a separate analysis is conducted for each component.

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{Figures/Dot Plot - Combined.pdf}
\caption{Fabric -- Key resource utilization for different request rates.}
\label{fig:Scatter_resources}
\end{figure}


\subsubsection{\textbf{CPU}}
\label{cpu}

The analysis begins by focusing on the average \ac{CPU} utilization across a 14-second period, with a subsequent focus on more detailed time intervals. We observe that as the request rate increases, the linear correlation between the request rate and CPU utilization of peers breaks at \ac{freq}=1600\,s$^{-1}$, indicating a potential saturation point or limitation in \ac{CPU} capacity. This poses a potential bottleneck that requires further examination. 

Looking into the CPU usage across all individual cores (Figure~\ref{fig:Boxplot_all CPUs}) reveals limited utilization across orderers and clients that is not plateauing at higher request rates. Focusing on peers, we observe a significant variance in \ac{CPU} utilization among peers, ranging from 25\% to 80\% at higher request rates. Such variability could be an indicator that the network is distributing its resources unevenly, with some peers carrying more workload than others, or reflect an uneven allocation between nodes’ cores.

\begin{figure}
     \centering
     \makebox[\columnwidth]{\includegraphics[width=0.75\columnwidth, trim=0cm 0cm 0cm -0.5cm, clip]{Figures/cpu_all_cores_plot.pdf}}
     \caption{Fabric -- CPU utilization of all cores.}
     \label{fig:Boxplot_all CPUs}
\end{figure}

First, we investigate the CPU utilization per peer in Figure~\ref{fig:CHART_workload distribution_peer_CPU_absolute_agg=mean}, which suggests an equitable distribution of computational resources among the peers, with all of them showing comparable levels of computational effort, with peer~5 falling behind slightly. Subsequently, the investigation shifts to analyzing the mean \ac{CPU} utilization of individual cores for a single peer (peer~0 in this case) in Figure~\ref{fig:CHART_workload distribution_peer0 processors}. It is apparent that this also is not the cause of the high fluctuations in \ac{CPU} usage since all cores indicate similar utilization.

\begin{figure}
    \subfloat[Mean utilization per peer.\label{fig:CHART_workload distribution_peer_CPU_absolute_agg=mean}]{{\includegraphics[width=0.5\linewidth]{Figures/mean_util_peer_plot.pdf}}}
    \subfloat[Mean utilization of peer~0 per core.\label{fig:CHART_workload distribution_peer0 processors}]{{\includegraphics[width=0.5\linewidth]{Figures/mean_util_core_plot_peer0.pdf}}}
    \caption{Fabric -- peer mean CPU utilization.}
    \label{fig:CPU utilization in peers}
\end{figure}

Following the inconclusive results of both possible explanations, the analysis progresses to evaluate the temporal evolution of \ac{CPU} usage across individual cores at the highest \ac{freq} before the utilization plateaus (Figure~\ref{fig:Chart_timeline_peer0 processors freq=1600}). This \ac{freq} represents the peak stress on the network prior to any performance degradation. Here, we observe that individual cores can fluctuate as much as 30\,\% within a single run. At this point, this analysis comes to a halt as it is impossible to deduce the reasons behind these fluctuations from \ac{CPU} utilization data only. However, the mean utilization illustrates that these fluctuations balance themselves out over time, with all cores clocking in at a similar average. This suggests that the high fluctuations in \ac{CPU} usage are not the reason behind the plateauing.


It is also worth noting that from Figure~\ref{fig:CPU utilization in peers}, we see that average \ac{CPU} usage plateaus at around 50\,\% across all cores on all peers. This marks a significant improvement to the prior versions of Fabric. However, it is important to highlight that in scenarios utilizing a higher number of vCPUs (16~in our case), Fabric~v2.0 still has a mediocre mean utilization for a resource that can limit the entire system, which leaves room for further improvement. 

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth, trim=0cm 0cm 0cm -1.8cm, clip]{Figures/util_time_plot_peer0_1600.pdf}

    \caption{Fabric -- CPU utilization of peer~0 for \ac{freq}=1600\,s$^{-1}$.}
    \label{fig:Chart_timeline_peer0 processors freq=1600}
\end{figure}


\subsubsection{\textbf{Network}}
\label{network}

The network-related part of the analysis begins by looking into the mean network utilization, distinguishing between inbound and outbound traffic for the different types of nodes. Unsurprisingly, there is a strong correlation between the request rate and mean traffic.
In the examination of orderers, we observe that both incoming and outgoing traffic do not plateau at high request rates, suggesting that they are not the bottleneck (Figure~\ref{fig:workload distribution_orderer_network_absolute}). Notably, orderer~0 broadcasts a disproportionate amount of traffic compared to the rest, which indicates that orderer~0 is the leader in \ac{raft} consensus and, as a result, has the additional task of broadcasting new blocks to each following orderer. In our experiments, we did not simulate crashing nodes, so orderer~0 remained the leader for the whole duration of the experiments (cf.~\cite{guggenberger_-depth_2022}), making this discrepancy logical. 


A more detailed analysis of the network traffic allows its decomposition into individual components, such as the traffic generated by block propagation. According to Fabric's architecture, the outbound traffic of followers among orderers predominantly consists of sending blocks to the peers, and from Figure~\ref{fig:workload distribution_orderer_network_absolute}, an overlapping between inbound and outbound traffic of the followers is observed. The overlapping traffic, combined with the fact that followers receive each block once from the leader, suggests that each orderer forwards the received block only once.
To evaluate the validity of this hypothesis, we compare followers' outbound traffic with the leader's outbound traffic (Figure~\ref{fig:workload distribution_orderer_network out - leader durch follower}). The ratio consistently stands around four, aligning with our hypothesis and the Fabric architecture where the \ac{raft} leader distributes the block to each follower, accounting for three times in our case and an additional time to a peer, totaling four times. 
Our analysis does not take into consideration the traffic generated by consensus-related messages, such as appended entries or heartbeat messages~\cite{Fabric_config}, since differentiation between them and the traffic from block propagation is challenging. Nonetheless, the consensus-related messages generate significantly less traffic compared to block dissemination, and as a result, we expect that the outbound traffic of follower orderers provides a viable approximation for assessing the traffic associated with block propagation.

\begin{figure}
\subfloat[Mean utilization per orderer\\(inbound traffic of orderer~1,~2,~3 \\ overlaps with their outbound traffic).\label{fig:workload distribution_orderer_network_absolute}]{{\includegraphics[width=0.5\linewidth]{Figures/inbound_outbound_orderer_plot.pdf} }}
\subfloat[Ratio of leader outbound traffic over follower outbound traffic.\label{fig:workload distribution_orderer_network out - leader durch follower}]{{\includegraphics[width=0.5\linewidth]{Figures/ratio_network_plot.pdf} }}

\caption{Fabric -- orderer mean network utilization (outbound traffic as continuous and inbound traffic as dashed lines).}
\label{fig:network for orderers}
\end{figure}

Regarding peers (Figure~\ref{fig:network for peers}), we see that inbound traffic scales linearly with the \ac{freq} for all of them. This uniformity aligns with the architecture in our experiment, as all peers receive the same number of transaction proposals (i.e., endorsement requests) from clients and the same number of blocks. Additionally, inbound traffic scales linearly throughout the experiment, indicating it's not a bottleneck.
Concerning outbound traffic, we observe that it plateaus for some peers while remaining unaffected for others (Figure~\ref{fig:workload distribution_peer_network_absolute}). This divergence allows for the classification of peers into two main clusters, color-coded as blue and orange, based on their outbound traffic. The two groups distribute communication workload differently, with blue peers registering more than twice the sent data of the orange peers. The blockchain's architecture explains this divergence since blue peers are the gossip leaders of their respective organizations, with one gossip follower each. For instance, organization~0 consists of orderer~0, peer~0, and peer~1, with peer~0 acting as the anchor peer. As such, peer~0 receives all new blocks from orderer~0 and forwards them to peer~1.


The primary distinction in outbound traffic among peers stems from the block propagation between them. To confirm that blue peers correspond to gossip leaders and the accuracy of previous assumptions regarding traffic generated by block propagation, we perform a further analysis by deducting the traffic associated with block propagation, as obtained from the previous analysis of the ordering service, from the total outbound traffic of gossip leader peers (Figure~\ref{fig:plot_network_traffic_peer_no_block}).
The resulting traffic is relatively uniform across all peers, confirming that the blue peers are the gossip leaders. Furthermore, we observe a significant overlap in outbound traffic among peers, particularly at lower request frequencies, while some discrepancies exist at higher rates. This is expected as traffic stemming from consensus messages increases at higher request rates, making our approximation less accurate. The outbound traffic of peers consists of sending requested endorsements and confirmations that requested transactions have been committed to the blockchain to clients. Since the outbound traffic of peers plateaus at high \ac{freq}, it suggests that these components are potential bottlenecks.


To pinpoint the specific bottleneck, we focus on client traffic (Figure~\ref{fig:network for peers, orderers and clients}). The inbound traffic of clients, although it exhibits a drop at higher request rates, is generated by the same components as the outbound traffic of peers, leaving us with the same potential bottlenecks as before. The outbound traffic of clients is comprised of transaction proposals submitted to peers and endorsed transactions sent to the orderers. Since the traffic does not plateau, it suggests that none of them is the bottleneck.
Overall, we have seen that the traffic generated by the endorsed transactions the clients send to the ordering service and the traffic generated by the blocks the service sends to the peers never plateaus. This indicates that the execution and ordering phases are not the bottleneck. Since the endorsements that peers send back to the clients come in between the execution and ordering phases, this suggests that they are not the bottleneck, leaving us only with the transaction confirmations that peers send to clients as the possible culprit. These are sent after the validation phase, suggesting that this remains the primary bottleneck even in Fabric v2.0.


\begin{figure}
\subfloat[Mean utilization per peer.\label{fig:workload distribution_peer_network_absolute}]{{\includegraphics[width=0.5\linewidth]{Figures/inbound_outbound_peer_plot.pdf} }}
\subfloat[Outbound traffic per peer excluding traffic generated by block propagation.\label{fig:plot_network_traffic_peer_no_block}]{{\includegraphics[width=0.5\linewidth]{Figures/plot_network_traffic_peer_no_block.pdf} }}
\caption{Fabric -- peer mean network utilization (outbound traffic as continuous and inbound traffic as dashed lines).}
\label{fig:network for peers}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.725\linewidth]{Figures/inbound_outbound_client_plot.pdf} 

    \caption{Fabric -- Client mean network utilization (outbound traffic as continuous and inbound traffic as dashed lines).}
    \label{fig:network for peers, orderers and clients}
\end{figure}



\subsubsection{\textbf{Memory \& Hard Drive}}
\label{memory}

From Figure~\ref{fig:Scatter_resources}, we see that the utilization of memory and hard drive is limited, indicating that neither of them is the bottleneck. Despite this, we examine the resource utilization of peers and orderers further. We do not examine clients since their utilization remains unaffected by the increasing number of requests. 
Starting with memory usage (Figure~\ref{fig:memory_utilisation}), we see peers and orderers exhibit low and non-plateauing usage levels, suggesting that memory constraints are not the bottleneck. We observe some minor differences in memory utilization across orderers, but given the low overall utilization, it is highly unlikely that they constitute a bottleneck, and we don't investigate them further.


Moving to hard drive utilization (Figure~\ref{fig:i_o_utilisation}), we observe that the orderers' usage is increasing linearly with the \ac{freq} and, as a result, likely does not pose a problem. Most peers' I/O operations (such as ledger updates or block processing) occur during or after the validation phase. As a result, even though their utilization plateaus, it does not provide us with any new information. Additionally, due to the variety in read/write operations that peers execute, it is impossible to differentiate between them with only data related to resource utilization at hand. Moreover, with the peak utilization at approximately 1~\%, it is evident that hard drive usage is far from reaching capacity, pointing out that constraints lie within a different component, which in turn limits hard drive utilization.

As mentioned in Section ~\ref{sec:background}, the validation phase is comprised of three steps: \ac{vscc}, \ac{mvcc}, and each peer updating its database. As the peers' hard drive utilization is minimal, this leaves only \ac{vscc} and \ac{mvcc} as the potential bottlenecks in the validation phase.


\begin{figure}
 \subfloat[Mean utilization per peer\label{fig:memory_usage_peer}]{{\includegraphics[width=0.5\linewidth]{Figures/plot_peer_memory_usage.pdf} }}
 \subfloat[Mean utilization per orderer\label{fig:memory_usage_orderer}]{{\includegraphics[width=0.5\linewidth]{Figures/plot_orderer_memory_usage.pdf} }}

\caption{Fabric -- Mean memory utilization.}
\label{fig:memory_utilisation}
\end{figure}


\begin{figure}
 \subfloat[Mean utilization per peer\label{fig:i_o_usage_peer}]{{\includegraphics[width=0.5\linewidth]{Figures/peer_mean_io_plot.pdf} }}
 \subfloat[Mean utilization per orderer\label{fig:i_o_usage_orderer}]{{\includegraphics[width=0.5\linewidth]{Figures/orderer_mean_io_plot.pdf} }}

\caption{Fabric -- Mean hard drive utilization.}
\label{fig:i_o_utilisation}
\end{figure}



\subsection{Fabric: Throughput}
\label{throughput}

In the second part of our analysis, we attempt to find correlations between Fabric's throughput and the components highlighted as potential bottlenecks in the first part, namely peer \ac{CPU} utilization and peer network traffic. 
We start by gaining an overview of how the request rate affects throughput. This is achieved by plotting the throughput as a rolling mean across different window sizes (Figure~\ref{fig:throughput_windows}). A one-second window size results in each data point being plotted individually, revealing how unstable the throughput of this Fabric network gets beyond \ac{freq}=1200\,s$^{-1}$, with fluctuations in \ac{fresp} reaching up to 1000\,s$^{-1}$ within a single run. To see the overall network performance trend, we increase the window size, taking 3~cases at 3~seconds, 8~seconds, and full run. In these cases, the mean is calculated over more data points, and outliers are smoothed out. Here, we see that, on average, the system keeps up with the request rate until reaching approximately \ac{freq}=1600\,s$^{-1}$. Beyond this point, the interrelationship breaks, marking this as the peak throughput observed in the experiment.

\begin{figure}
 \subfloat[1s window\label{fig:window_1s}]{{\includegraphics[width=0.5\linewidth]{Figures/tx_request_response_window_1s.pdf} }}
 \subfloat[3s window\label{fig:window_3s}]{{\includegraphics[width=0.5\linewidth]{Figures/tx_request_response_window_3s.pdf}}}

  \subfloat[8s window\label{fig:wwindow_8s}]{{\includegraphics[width=0.5\linewidth]{Figures/tx_request_response_window_8s.pdf} }}
 \subfloat[15s window\label{fig:window_14s}]{{\includegraphics[width=0.5\linewidth]{Figures/tx_request_response_txs_received.pdf}}}

\caption{Fabric -- Rolling mean of throughput with different window sizes.}
\label{fig:throughput_windows}
\end{figure}

To obtain insights into the link between peer \ac{CPU} utilization and network traffic, we examine Figure~\ref{fig:throughput vs CPU vs Network}, which plots the two resources against the network's throughput employing a rolling average with a 3-second window. We selected this interval as it matches the average duration required for a transaction to be committed to the blockchain under high request rates. This is significant because queuing effects become prominent at elevated \ac{freq}, and opting for a shorter time window could underestimate throughput.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/CPU & Traffic - Throughput.pdf} 

    \caption{Fabric -- Throughput against key resources.}
    \label{fig:throughput vs CPU vs Network}
\end{figure}

For \ac{CPU} usage, we observe an initial linear increase with throughput until the characteristic plateau is reached. Both variables seem to increase at a similar rate at the beginning, implying that increased throughput proportionally strains the \ac{CPU}. Additionally, we observe that the instability in \ac{CPU} utilization starts at around \ac{fresp}=1200\,s$^{-1}$, which is also the point at which the correlation between \ac{freq} and \ac{fresp} starts breaking down (Figure~\ref{fig:window_1s}). This indicates that \ac{CPU} usage is more closely correlated to throughput than to the request rate. Similarly, although network traffic increases with throughput, it does so at a lower rate and begins to exhibit instability already at around \ac{fresp}=600\,s$^{-1}$, where the throughput still manages to keep up with the request rate. 

Digging deeper, we focus on the throughput of individual peers (Figure~\ref{fig:throughput per peer}). Here, we see that every peer contributes similarly to the overall throughput, with all of them moving in unison with minor variations at high \ac{freq}. Given our findings in Section~\ref{network}, where we noted significant differences in network traffic between gossip leaders and followers, this outcome suggests that network traffic is not a significant factor in determining throughput compared to \ac{CPU} utilization. If it were, we would expect noticeable differences in throughput between gossip leaders and followers. Consequently, this leaves us with peer \ac{CPU} utilization as the primary factor behind throughput leveling off.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth, trim=0cm 0cm 0cm -2.1cm, clip]{Figures/mean_response_peer_plot.pdf} 

    \caption{Fabric -- Throughput per peer.}
    \label{fig:throughput per peer}
\end{figure}

The crucial role of peer CPU utilization further supports the findings in Section~\ref{resource_util} that \ac{vscc} and \ac{mvcc} are the main bottlenecks in Fabric as both depend on peer \ac{CPU}. Given that validations in \ac{vscc} are parallelized and we have noted that the mean core utilization is limited and mean \ac{CPU} utilization is similar across all peers, it appears that the main bottleneck is \ac{vscc}. However, the sequential execution of concurrency controls in \ac{mvcc}, combined with the fluctuating utilization per core featured in Figure~\ref{fig:Chart_timeline_peer0 processors freq=1600}, makes it impossible to determine its role as a bottleneck. As a result, while \ac{vscc} appears to be the main culprit, we cannot conclusively confirm this with the available data. This also highlights a shortcoming of the \ac{dlps}' resource utilization-based approach, which was chosen to make it blockchain agnostic. However, as a trade-off for this generalized approach, the resulting data are less specific than they could be. Therefore, further research would require taking into account and evaluating more precise monitoring data, e.g., using SoundCloud’s Prometheus that is incorporated in Fabric~\cite{Fabric-prometheus}.





















\subsection{Quorum: Resource utilization}
\label{resource_util_quorum}

The Quorum analysis, as before, starts by gaining an overview of the four resources in relation to \ac{freq} (Figure~\ref{fig:q_Scatter_resources}). To analyze Quorum's performance in more detail, we refine our analysis by increasing the request rate in increments of 100~requests per second. As with the case of Fabric, even at this early stage, it is apparent that \ac{CPU} and network utilization are closely correlated with the request rate. Memory and hard drive usage are limited, with I/O operations exhibiting high fluctuations but generally registering less than 1~\% usage. Across all resources, client utilization appears to be minimal, and it is either unaffected or grows linearly with the request rate. As a result, in the following sections, we concentrate on the resource utilization of nodes.

\begin{figure}
\centering
\includegraphics[width=1\linewidth]{Figures/q_dot_plot.pdf}
\caption{Quorum -- Key resource utilization for different request rates \ac{freq}.}
\label{fig:q_Scatter_resources}
\end{figure}


\subsubsection{\textbf{CPU}}
\label{q_cpu}

We start the \ac{CPU} analysis by looking into the utilization across all cores, where again we note significant fluctuations among the nodes as the request rates increase (Figure~\ref{fig:q_cpu_all_cores}). Examining the mean node \ac{CPU} utilization (Figure~\ref{fig:cpu_util_per_node}), we see that nodes can be grouped into three distinct categories. Node~0~(green) consistently exhibits the highest utilization across all request rates, indicating it is the \ac{raft} leader. This is attributed to the leader's additional operations, such as transaction ordering and compiling transactions into a block. Nodes~1,~2,~and~3~(blue) display slightly lower utilization levels, indicating their role in receiving and pre-validating transactions alongside node~0. In contrast, the remaining nodes (orange) exhibit significantly lower \ac{CPU} usage, with their primary role being the appending of blocks to their local version of the blockchain.


Examining the utilization per core of node~0 (Figure~\ref{fig:q_mean_util_core}) we observe that one core (core~15) bears a higher workload across all request rates. This is due to the fact that with the exception of pre-validation, all other tasks of the leader are executed sequentially, leading to a disproportionate strain on one core. Following this, we examine the temporal evolution of \ac{CPU} usage across individual cores at \ac{freq}=2300\,s$^{-1}$, which is the highest request rate before \ac{CPU} utilization plateaus (Figure~\ref{fig:q_cpu_freq}). Here, we see fluctuations by as much as 20\,\% for both the leader and the follower, with disparities of up to 10\,\% between individual cores, excluding core~15 for node~0. Notably, the main difference between the mean utilization of node~0 and nodes1,~2,~and~3 comes only from core~15. These results suggest that parallel processing in Quorum is even more limited than that of Fabric, with each core's average usage not exceeding 40\,\% and specific tasks of the leader burdening only one core.


With respect to bottleneck detection, nodes~0,~1,~2,~and~3 reach an apparent plateau at \ac{freq}=2400\,s$^{-1}$, while for the remaining nodes, some of them plateau while others do not. Additionally, we observe that there is a considerable decrease in \ac{CPU} usage at \ac{freq}=1800\,s$^{-1}$, which, even though it does not necessarily indicate a bottleneck, could provide clues for identifying factors contributing to the decline in \ac{CPU} utilization. 
From Figure~\ref{fig:cpu_util_per_node}, we observe that node~0 and nodes~1,~2,~and~3 show similar behavior after reaching a plateau. This similarity suggests that transaction ordering and block building, which are the main unique operations performed by the leader, are likely not the sources of the bottleneck. If they were, we would expect the leader's utilization pattern to diverge from that of the other nodes after the plateau. Examining Figure~\ref{fig:q_mean_util_core}, we see a rapid decline in the utilization of core~15 at high request rates. Considering that the remaining sequential operations, such as ordering the transactions, committing the block to the chain, and propagating it through the nodes, typically require minimal \ac{CPU} resources, this sharp drop cannot be justified by these processes, and it appears that another component limits \ac{CPU} utilization. 

\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{Figures/q_cpu_all_cores_plot.pdf}
\caption{Quorum -- CPU utilization of all cores.}
\label{fig:q_cpu_all_cores}
\end{figure}


\begin{figure}
 \subfloat[Mean utilization per Node.\label{fig:cpu_util_per_node}]{{\includegraphics[width=0.5\linewidth]{Figures/q_mean_util_peer_plot.pdf} }}
 \subfloat[Mean utilization of Node~0 per core.\label{fig:q_mean_util_core}]{{\includegraphics[width=0.5\linewidth]{Figures/mean_util_core_plot_node0.pdf}}}
\caption{Quorum -- Mean CPU utilization.}
\label{fig:q_cpu_util}
\end{figure}


\begin{figure}
 \subfloat[Node~0.
 \label{fig:q_utiil_node0}]
 {{\includegraphics[width=0.5\linewidth]{Figures/q_util_time_plot_node0_2300.pdf}}}
 \subfloat[Node~1.
 \label{fig:q_util_node1}]
 {{\includegraphics[width=0.5\linewidth]{Figures/q_util_time_plot_node1_2300.pdf}}}
\caption{Quorum -- CPU utilization for \ac{freq}=2300\,s$^{-1}$.}

\label{fig:q_cpu_freq}
\end{figure}


\subsubsection{\textbf{Network}}
\label{q_network}

Continuing the analysis by looking into the mean network utilization of the nodes (Figure~\ref{fig:q_network_nodes}), we can categorize the nodes into three groups as before. Due to the complexity of the Quorum network traffic, we are not able to decompose the traffic into individual components with adequate accuracy. Therefore, we rely entirely on the architectural design to identify the reasons behind the plateau. As with the case of Fabric, the network analysis does not take into consideration the traffic generated by consensus messages since they generate minimal traffic.

Starting with the blue nodes, we note that their outbound traffic levels off at \ac{freq}=2400\,s$^{-1}$ while signs of plateauing in their inbound traffic appear at \ac{freq}=1800\,s$^{-1}$. The inbound traffic primarily consists of transactions received either directly from clients or through gossip and blocks from the leader, whereas their outbound traffic originates from the dissemination of pre-validated transactions. This suggests that these operations are the limiting factors at their respective request rates.
While we see similar patterns for the orange nodes, the patterns of the leader are essentially the opposite of those of other nodes. The inbound traffic is comprised of all the transactions that are broadcasted to the network and reach the leader through gossip or directly from the clients, and plateaus at \ac{freq}=2400\,s$^{-1}$. The outbound traffic involves mainly block dissemination to the other nodes and plateaus at \ac{freq}=1800\,s$^{-1}$. Since their inbound traffic plateaus at \ac{freq}=2400\,s$^{-1}$, it indicates that the leader keeps receiving the transactions from the blue nodes normally up until that point, leaving us only with block dissemination as the main bottleneck at \ac{freq}=1800\,s$^{-1}$ and transaction propagation as the main issue for \ac{freq}=2400\,s$^{-1}$.


Combining our findings with \ac{CPU} utilization findings, the rapid drop in \ac{CPU} utilization for core~15 at \ac{freq}=2400\,s$^{-1}$ (Figure~\ref{fig:q_mean_util_core}) is caused because the leader does not receive enough transactions from the other nodes and not because the \ac{CPU} cannot keep up with the processes. At \ac{freq}=1800\,s$^{-1}$, the decline could be attributed to either the block propagation or one of the processes preceding it, such as transaction pre-validation and adding the block to the chain, since we already excluded transaction ordering and block building as potential bottlenecks in Section~\ref{q_network}. Considering appending the block to the blockchain is not \ac{CPU} intensive, the primary issues likely lie with block propagation or pre-validation. Using the same line of reasoning for the \ac{freq}=2400\,s$^{-1}$ rate, the bottleneck appears to be either transaction propagation, as already identified, or pre-validation, as it is the only operation that precedes propagation.


\begin{figure}
\centering
\includegraphics[width=0.5\linewidth, trim=0cm 0cm 0cm -1.6cm, clip]{Figures/q_inbound_outbound_node_plot.pdf}
\caption{Quorum -- Node mean network utilization (outbound traffic as continuous and inbound traffic as dashed lines).}
\label{fig:q_network_nodes}
\end{figure}

\subsubsection{\textbf{Memory \& Hard Drive}}
\label{q_m&h}

Similar to our observations with Fabric, Figure~\ref{fig:q_Scatter_resources} indicates that neither memory nor hard drive utilization are likely to be bottlenecks. Nevertheless, we proceed to examine the utilization metrics of the nodes. The analysis reveals consistent behavior in memory utilization across all nodes, with no signs of plateauing (Figure~\ref{fig:q_memory}). This uniformity suggests that memory is not contributing to performance degradation. Despite observing significant peaks in hard drive utilization in Figure~\ref{fig:q_Scatter_resources}, the mean utilization remains below 1\,\% (Figure~\ref{fig:q_io}), indicating it is not a constraining factor either. The large fluctuations are probably related to the writing of the block into each node's database, but since it is improbable that it leads to a bottleneck, we desist from further investigations.

\begin{figure}
 \subfloat[Memory utilization.\label{fig:q_memory}]{{\includegraphics[width=0.5\linewidth]{Figures/q_plot_peer_memory_usage.pdf} }}
 \subfloat[Hard drive utilization.\label{fig:q_io}]{{\includegraphics[width=0.5\linewidth]{Figures/q_peer_mean_io_plot.pdf}}}
\caption{Quorum -- Mean utilization per node.}
\label{fig:q_memory_util}
\end{figure}

Concluding the first part of the Quorum analysis, we identify two primary points where there is a significant drop in performance. The first one appears at \ac{freq}=1800\,s$^{-1}$, with the main factors likely being block propagation or the pre-validation of transactions. The second one is observed at \ac{freq}=2400\,s$^{-1}$, which appears to stem from the propagation of transactions through the network or the pre-validation of transactions.


\subsection{Quorum: Throughput}
\label{q_throughput}

The throughput analysis of Quorum starts by examining its correlation with the request rate. We see that even for small window sizes, throughput remains relatively stable but starts to exhibit higher fluctuations at \ac{freq}=1800\,s$^{-1}$. Examining the full run, we observe that throughput plateaus at around \ac{fresp}=2100\,s$^{-1}$, which is significantly lower than the maximum request rate. This suggests that the overall performance of the blockchain started to decline long before reaching the highest request rate. This observation suggests that the performance degradation noted at \ac{freq}=1800\,s$^{-1}$ for both \ac{CPU} and network utilization may be more critical in identifying the bottleneck.

\begin{figure}
 \subfloat[1s window\label{fig:q_window_1s}]{{\includegraphics[width=0.5\linewidth]{Figures/q_tx_request_response_window_1s.pdf} }}
 \subfloat[3s window\label{fig:q_window_3s}]{{\includegraphics[width=0.5\linewidth]{Figures/q_tx_request_response_window_3s.pdf}}}

  \subfloat[8s window\label{fig:q_window_8s}]{{\includegraphics[width=0.5\linewidth]{Figures/q_tx_request_response_window_8s.pdf} }}
 \subfloat[15s window\label{fig:q_window_14s}]{{\includegraphics[width=0.5\linewidth]{Figures/q_tx_request_response_txs_received.pdf}}}

 \caption{Quorum -- Rolling mean of throughput with different window sizes.}
\label{fig:q_throughput_windows}
\end{figure}

Examining throughput against the \ac{CPU} and network utilization (Figure~\ref{fig:q throughput vs CPU vs Network}), we see similar growth rates and patterns. Both resources keep up with throughput at the beginning and experience higher performance fluctuations at around \ac{fresp}=1800\,s$^{-1}$. Beyond this point, the differences in throughput between request rates become less pronounced, becoming indistinguishable as it approaches \ac{fresp}=2100\,s$^{-1}$.

Since both resources exhibit similar patterns, we search for a common source behind the blockchain's performance degradation. Considering that block and validated transaction propagation are network-related, if they were the bottleneck, they would mainly impact network traffic. As a result, they are less likely to be the bottleneck. This leaves only transaction pre-validation as the possible constraining factor, which can impact both \ac{CPU} and network as it represents the first step in processing a transaction.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]
    {Figures/q_throughput_cpu_network.pdf} 

    \caption{Quorum -- Throughput against key resources.}
    \label{fig:q throughput vs CPU vs Network}
\end{figure}


Looking further into pre-validation, we deduce that the bottleneck is either pre-validation itself, i.e., the nodes do not validate the incoming transactions fast enough, which in turn slows down the network, or the nodes do not receive enough transactions. From  Figure~\ref{fig:q_Scatter_resources}, we see that the network utilization of clients increases linearly with the request rate, which suggests that they send the proper number of transactions to the nodes. 
Examining further the interaction of nodes with the incoming transactions, we look into the number of rejected transactions (Figure~\ref{fig:rejected_txs}). By the term rejected transactions, we refer to those transactions that nodes decline to propagate through the network, resulting in clients receiving almost immediate (within less than 50ms) notification of transaction failure after submission. Initially, the count of rejected transactions remains minimal but begins to surge at \ac{freq}=1800\,s$^{-1}$, culminating in approximately 7000 rejections by \ac{freq}=2500\,s$^{-1}$. This escalation translates to a rejection rate of 14\,\%  before reaching a plateau. This significant increase in rejections prompts us to investigate further to understand the underlying causes.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth, trim=0cm 0cm 0cm -2cm, clip]{Figures/q_rejected txs.pdf} 

    \caption{Quorum -- Mean number of rejected transactions.}
    \label{fig:rejected_txs}
\end{figure}

In Quorum, transactions are categorized as either executable or non-executable. Executable transactions are the ones that can be immediately included in a block, while non-executable transactions are out of nonce order and must wait for preceding transactions with lower nonce to execute first. Investigating the reasons behind the increasing rejection rates, we identify two main constraints in Quorum's transaction handling. First, Quorum caps the transaction pool at 4096~executable and 10000~non-executable transactions~\cite{noauthor_quorumcmdutilsflagsgo_nodate}. However, according to Figure~\ref{fig:q_full_pool}, the transaction pool's capacity is never fully utilized, suggesting that this is not the cause behind the rejections. The periodic drop in the number of transactions in the pool aligns with the end of each ramp-up phase of DLPS, where nodes commit pending transactions to blocks and clear the pool before the new ramp-up commences.

The second limitation involves the clients, who are limited to 16~executable and 500~non-executable transactions in the pool at any given time~\cite{noauthor_quorumcmdutilsflagsgo_nodate}. Examining Figure~\ref{fig:q_client_pool}, we see that at \ac{freq}=1800\,s$^{-1}$, transaction submission by six clients begins to exhibit instability, diverging from the previous linear relationship with the request rate, and most clients diverge at \ac{freq}=2400\,s$^{-1}$. This pattern suggests that clients are reaching the limit of executable transactions in the pool, leading to an increased rate of rejections. To answer this definitively, we would have to separate the client transactions into executable and non-executable and examine which type is getting rejected, something that is not possible due to \ac{dlps}' blockchain agnostic nature that does not allow us to distinguish transactions between the different types. However, considering that the number of rejected transactions increases sharply at \ac{freq}=1800\,s$^{-1}$, combined with the observed reduction in \ac{CPU} and network utilization starting at the same point and the subsequent plateau at \ac{freq}=2400\,s$^{-1}$, strongly suggest that the primary bottleneck is the limit on the number of executable transactions per client.

\begin{figure}
 \subfloat[Cumulative number of transa-\\ctions in the pool.
 \label{fig:q_full_pool}]
 {{\includegraphics[width=0.5\linewidth]{Figures/q_txs_in_pool.pdf} }}
 \subfloat[Number of transactions in the\\ pool per client.
 \label{fig:q_client_pool}]
 {{\includegraphics[width=0.5\linewidth]{Figures/q_txs_client_in_pool.pdf}}}
\caption{Quorum -- Transactions in the pool.}
\label{fig:q_pool}
\end{figure}







